Cloning Games: A General Framework for Unclonable Primitives

The powerful no-cloning principle of quantum mechanics can be leveraged to achieve interesting primitives, referred to as unclonable primitives, that are impossible to achieve classically. In the past few years, we have witnessed a surge of new unclonable primitives. While prior works have mainly focused on establishing feasibility results, another equally important direction, that of understanding the relationship between different unclonable primitives is still in its nascent stages. Moving forward, we need a more systematic study of unclonable primitives. To this end, we introduce a new framework called cloning games. This framework captures many fundamental unclonable primitives such as quantum money, copy-protection, unclonable encryption, single-decryptor encryption, and many more. By reasoning about different types of cloning games, we obtain many interesting implications to unclonable cryptography, including the following: 1. We obtain the first construction of information-theoretically secure single-decryptor encryption in the one-time setting. 2. We construct unclonable encryption in the quantum random oracle model based on BB84 states, improving upon the previous work, which used coset states. Our work also provides a simpler security proof for the previous work. 3. We construct copy-protection for single-bit point functions in the quantum random oracle model based on BB84 states, improving upon the previous work, which used coset states, and additionally, providing a simpler proof. 4. We establish a relationship between different challenge distributions of copy-protection schemes and single-decryptor encryption schemes. 5. Finally, we present a new construction of one-time encryption with certified deletion.

==> prelims_cp.tex <==
\newcommand{\fclass}{\mathcal{F}}
\newcommand{\distrclass}{\mathfrak{D}_X}
\newcommand{\pirateexp}[4]{\mathsf{PirExp}^{#1,#2}_{#3,#4}}
\newcommand{\trivialprob}{p^\mathsf{triv}}
\newcommand{\prob}{\mathsf{Pr}}

\subsection{Copy-Protection}
\label{sec:prelims_cp}
Below we present the definition of a copy-protection scheme.
\begin{definition} [Copy-Protection Scheme] \label{def:copyprotection}
 Let $\fclass = \fclass(\secparam)$ be a class of efficiently computable functions of the form $f: X \to Y$. A copy protection scheme for $\fclass$ is a pair of QPT algorithms $(\copyprotect, \eval)$ such that: \begin{itemize}
    \item \textbf{Copy Protected State Generation:} $\copyprotect(1^\secparam, d_f)$ takes as input the security parameter $1^\secparam$ and a classical description $d_f$ of a function $f \in \fclass$ (that efficiently computes $f$). It outputs a mixed state $\rho_f \in \density{Z}$, where $Z$ is the output register.
    \item \textbf{Evaluation:} $\eval(1^\secparam, \rho, x)$ takes as input the security parameter $1^\secparam$, a mixed state $\rho\in \density{Z}$, and an input value $x\in X$. It outputs a bipartite state $\rho' \otimes \ket{y}\bra{y} \in \density{Z} \otimes \density{Y}$.
    
\end{itemize}
\end{definition}

\noindent We will sometimes abuse the notation and write $\eval(1^\secparam, \rho, x)$ to denote the classical output $y \in Y$ when the residual state $\rho'$ is not significant.

\begin{definition}[Correctness] \label{def:cpcorrectness}
A copy-protection scheme $(\copyprotect,\eval)$ for $\fclass$ is \textbf{$\delta$-correct} if the following holds: for every $x \in X$, $f \in \fclass$,
$$\Pr \left[ f(x) \leftarrow \eval(1^\secparam, \rho_f,x)\ :\ \rho_f \leftarrow \copyprotect(1^{\secparam},d_f) \right] \geq \delta.$$
If $\delta \ge 1 - \negl(\secparam)$, we simply say that the scheme is \textbf{correct}.
\end{definition}

\begin{remark}
When $\delta$ is negligibly close to 1, the evaluation algorithm $\eval$ can be implemented so that it does not disturb the state $\rho_f$. This ensures that $\rho_f$ can be reused polynomially many times with arbitrary inputs.
\end{remark}

We define security via a piracy experiment.

\begin{definition}[Piracy Experiment]
\label{def:piracyexperiment}
A \textbf{piracy experiment} is a security game defined by a copy-protection scheme $(\cp, \eval)$ for a class of functions $\fclass$ of the form $f:X\to Y$, a distribution $\distr_\fclass$ over $\fclass$, and a class of distributions $\distrclass = \{\distrclass(f)\}_{f \in \fclass}$ over $X \times X$. It is the following game between a challenger and an adversary, which is a triplet of algorithms $\abc$: 
\begin{itemize}
    \item \textbf{Setup Phase:} The challenger samples a function $f\leftarrow \distr_\fclass$ and sends $\rho_f \leftarrow \cp(1^\secparam, d_f)$ to $\alice$.
    \item \textbf{Splitting Phase:} $\alice$ applies a CPTP map to split $\rho_f$ into a bipartite state $\rho_{BC}$; it sends the $B$ register to $\bob$ and the $\C$ register to $\charlie$. No communication is allowed between $\bob$ and $\charlie$ after this phase.
    \item \textbf{Challenge Phase:} The challenger samples $(x_B, x_C) \leftarrow \distrclass(f)$ and sends $x_B, x_C$ to $\bob, \charlie$, respectively. 
    \item \textbf{Output Phase:} $\bob$ and $\charlie$ output $y_B \in Y$ and $y_C \in Y$, respectively, and send to the challenger. The challenger outputs 1 if $y_B = f(x_B)$ and $ y_C = f(x_C)$, indicating that the adversary has succeeded, and 0 otherwise. 
\end{itemize}
The bit output by the challenger is denoted by $\pirateexp{\cp}{\eval}{\distr_\fclass}{\distrclass}(1^\secparam, \abc)$.
\end{definition}

As noted by \cite{CMP20}, the adversary can always succeed in this game with probability negligibly close to \[\trivialprob(\distr_\fclass, \distrclass) := \max_{E \in \bracC{B,C}} \E_{\substack{f \from \distr_\fclass \\ (x_B,x_C) \from \distrclass(f)}} \max_{y \in Y} \prob \bracS{y \given x_E} \]
by sending $\rho_f$ to $\bob$ and have $\charlie$ guess the most likely output $y$ given input $x_C$ (or vice versa). In other words, $\trivialprob$ is the success probability of optimal guessing strategy for one party $E \in \bracC{B,C}$ given only the test input $x_E$.

Bounding the success probability of the adversary is bounded by $\trivialprob$ captures the intuition that $\rho_f$ is no more helpful for simultaneous evaluation than a black-box program that could only be given to one party. 

\begin{definition}[Copy-Protection Security] \label{def:cpsecurity}
Let $(\cp, \eval)$ be a copy-protection scheme for a class $\fclass$ of functions $f:X \to Y$. Let $\distr_\fclass$ be a distribution over $\fclass$ and $\distrclass = \left\{\distrclass(f)\right\}_{f \in \fclass}$ a class of distributions over $X$. Then, $(\cp, \eval)$ is called $\left(\distr_\fclass,\distrclass\right)$-\textbf{secure} if there exists a negligible function $\negl$ such that any QPT adversary $\abc$ satisfies \[\prob \left[ b = 1\ :\ b \leftarrow \pirateexp{\cp}{\eval}{\distr_\fclass}{\distrclass}\left(1^\secparam, \abc\right)  \right] \le \trivialprob(\distr_\fclass, \distrclass) + \negl(\secparam) .\]

\end{definition}

\paragraph{Copy Protection for Point Functions}
A \textit{point function} $f_y: \bit^{m} \to \bit$ is of the form \begin{align*}
    f_{y}(x) = \begin{cases} 1, & x = y \\ 0, & x \ne y  \end{cases}.
\end{align*}

When dealing with point functions, the classical description of $f_y$ will simply be $y$, and accordingly the distribution $\distr_\fclass$ over point functions will be represented by a distribution $\distr = \distr_\secparam$ over $\bit^m$. Since copy protection is trivially impossible for a learnable distribution $\distr$, we are going to restrict our attention to unlearnable distributions. 

\begin{definition}[Copy-Protection Security for Point Functions]\label{def:cpsecurityforpf} Let $m = \poly(\secparam)$ and $\fclass$ be the class of point functions $f_y : \bit^m \to \bit$. Let $\distrclass = \bracC{\distrclass(f)}_{f \in \fclass}$ be a class of input distributions over $\bit^m \times \bit^m$. A copy protection scheme $(\cp, \eval)$ for $\fclass$ is called $\distrclass$-\textbf{secure} if there exists a negligible function $\negl$ such that $(\cp, \eval)$ is $(\distr_\secparam, \distrclass)$-\textbf{secure} for all unlearnable distributions $\distr_\secparam$ over $\bit^m$.
\end{definition}

